RayNet: A Simulation Platform for Developing Reinforcement Learning-Driven Network Protocols

Reinforcement Learning (RL) has gained significant momentum in the development of network protocols. However, RL-based protocols are still in their infancy, and substantial research is required to build deployable solutions. Developing a protocol based on RL is a complex and challenging process that involves several model design decisions and requires significant training and evaluation in real and simulated network topologies. Network simulators offer an efficient training environment for RL-based protocols, because they are deterministic and can run in parallel. In this paper, we introduce \textit{RayNet}, a scalable and adaptable simulation platform for the development of RL-based network protocols. RayNet integrates OMNeT++, a fully programmable network simulator, with Ray/RLlib, a scalable training platform for distributed RL. RayNet facilitates the methodical development of RL-based network protocols so that researchers can focus on the problem at hand and not on implementation details of the learning aspect of their research. We developed a simple RL-based congestion control approach as a proof of concept showcasing that RayNet can be a valuable platform for RL-based research in computer networks, enabling scalable training and evaluation. We compared RayNet with \textit{ns3-gym}, a platform with similar objectives to RayNet, and showed that RayNet performs better in terms of how fast agents can collect experience in RL environments.

==> literature-rl.tex <==
-------------------------------- Frameworks --------------------------------
https://github.com/tkn-tub/ns3-gym

https://github.com/hust-diangroup/ns3-ai

https://github.com/Sharif-Rezaie/RL-TCP 

https://github.com/20kaushik02/TCP-RL

source code from https://knowledgedefinednetworking.org/

-------------------------------- ---------- --------------------------------





-------------------------------- Caching --------------------------------

Multi-Agent Reinforcement Learning for Efficient Content Caching in Mobile D2D Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8629363
*Matlab*

Deep Reinforcement Learning-Based Edge Caching in Wireless Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8964499
*numerical results (matlab?)*

Deep Reinforcement Learning for Cooperative Content Caching in Vehicular Edge Computing and Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8879573
*Python to build a simulation environment for the vehicular edge caching system*

A deep reinforcement learning-based framework for content caching
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8362276
*numerical results (matlab?)*

VeSoNet: Traffic-Aware Content Caching for Vehicular Social Networks Using Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10070376
*some combination of tools including  OMNeT++ - appears to be a bespoke system - no source code is available nor any details of integration*

QoE-Driven Edge Caching in Vehicle Networks Based on Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9422164
*numerical results (matlab?)*

Intelligent Video Caching at Network Edge: A Multi-Agent Deep Reinforcement Learning Approach
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9155373
*MacoCache learning model using pytorch - bespoke*

A Deep Reinforcement Learning-Based Caching Strategy for Internet of Things
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9238811
*Python, tensorflow - bespoke*

Deep Reinforcement Learning Approaches for Content Caching in Cache-Enabled D2D Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8891760
*numerical results (matlab?)*

Optimal and Scalable Caching for 5G Using Reinforcement Learning of Space-Time Popularities
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8241758
*numerical results (matlab?)*

A Reinforcement-Learning Approach to Proactive Caching in Wireless Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8374824
*numerical results (matlab?)*

Deep-Reinforcement-Learning-Based Optimization for Cache-Enabled Opportunistic Interference Alignment Wireless Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8036259
*Python, tensorflow - bespoke*

Self-adaptive power control with deep reinforcement learning for millimeter-wave Internet-of-vehicles video caching
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9194445
*Python, tensorflow - bespoke*

Mobility-Aware Edge Caching and Computing in Vehicle Networks: A Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8447267
*tensorflow - bespoke*

Caching Transient Data for Internet of Things: A Deep Reinforcement Learning Approach
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8542696
*Python, tensorflow - bespoke*
-------------------------------- ---------- --------------------------------






---------------------------- Congestion Control ----------------------------
TCP-Drinc: Smart Congestion Control Based on Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8610116


QTCP: Adaptive Congestion Control with Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8357943


SmartCC: A Reinforcement Learning Approach for Multipath TCP Congestion Control in Heterogeneous Networks
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8790762


Learning-Based and Data-Driven TCP Design for Memory-Constrained IoT
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7536338


Improving TCP Congestion Control with Machine Intelligence
https://dl.acm.org/doi/pdf/10.1145/3229543.3229550

-------------------------------- ---------- --------------------------------






--------------------------------- Routing ----------------------------------

Routing in optical transport networks with deep reinforcement learning
* custom-built simulator *


Toward Packet Routing With Fully Distributed Multiagent Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9166753
* ad-hoc simulator - topology, packets *

Reinforcement Learning for Solving the Vehicle Routing Problem
https://arxiv.org/abs/1802.04240
* Monte Carlo simulation *

RL-Routing: An SDN Routing Algorithm Based on Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9171590
* Mininet-based emulation *

TIDE: Time-relevant deep reinforcement learning for routing optimization
* real world implementation?*

Network routing based on reinforcement learning in dynamically changing networks
* simple simulator has been designed to demonstrate the happenings inside a computer network. A network is fed into the simulator as an adjacency matrix*

Using feedback in collaborative reinforcement learning to adaptively optimize MANET routing
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=1420665
* ns-2 simulations - no further discussion - ad-hoc? *

A Deep-Reinforcement Learning Approach for Software-Defined Networking Routing Optimization
https://arxiv.org/pdf/1709.07080.pdf
* The OMNeT++ discrete event simulator (v4.6) [16, 17] was used throughout the experiment to obtain the network delay under given traffic and routing. *

Adaptive Routing for Sensor Networks using Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=4019984
*ad-hoc - numerical results?*

Online Vehicle Routing With Neural Combinatorial Optimization and Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8693516
* proposed neural network is modeled with PyTorch *

Deep reinforcement learning meets graph neural networks: Exploring a routing optimization use case
https://www.sciencedirect.com/science/article/pii/S0140366422003784
*We implemented the DRL+GNN solution described in Section 4 with Tensorflow [29] and evaluated it on an OTN network simulator implemented using the OpenAI Gym framework [30]. *

SINET: Enabling Scalable Network Routing with Deep Reinforcement Learning on Partial Nodes
https://dl.acm.org/doi/pdf/10.1145/3342280.3342317
*OMNeT++ - not much detail*

Experience-driven Networking: A Deep Reinforcement Learning based Approach (INFOCOM 2018)
https://arxiv.org/abs/1801.05757
* ns-3 simulations no further details *

EER-RL: Energy-Efficient Routing Based on Reinforcement Learning
https://www.hindawi.com/journals/misy/2021/5589145/
* MATLAB *

Routing for Crowd Management in Smart Cities: A Deep Reinforcement Learning Perspective
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8703471
* python bespoke simulator*

A Hybrid of Deep Reinforcement Learning and Local Search for the Vehicle Routing Problems
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9141401
* MATLAB *

DROM: Optimizing the Routing in Software-Defined Networks With Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8502806
* OMNeT++, keras, tensorflow - no further details *

Feature Engineering for Deep Reinforcement Learning Based Routing
https://ieeexplore.ieee.org/abstract/document/8761276
* ad-hoc simulator *

-------------------------------- ---------- --------------------------------





-------------------------------- Multimedia --------------------------------

RL-FEC – A Self-Contained Reinforcement Learning Code of FEC for ns-3
https://www.projectguideline.com/rl-fec-a-self-contained-reinforcement-learning-code-of-fec-for-ns-3/
https://github.com/yeliqseu/rl-fec

Learning-Based FEC for Non-Terrestrial Networks With Delayed Feedback
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9628079

QARC: Video Quality Aware Rate Control for Real-Time Video Streaming via Deep Reinforcement Learning
https://arxiv.org/pdf/1805.02482.pdf
*trace-based simulations*

Neural Adaptive Video Streaming with Pensieve
https://dl.acm.org/doi/pdf/10.1145/3098822.3098843
*To train its models, Pensieve uses simulations over a large corpus of network traces. Pensieve uses a fast and simple chunk-level simulator.*

Fast coding unit size decision based on deep reinforcement learning for versatile video coding
*reference software VTM 7.0*

Rate Control Method Based on Deep Reinforcement Learning for Dynamic Video Sequences in HEVC
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9088297
*HEVC reference software HM16.19 and tensorflow*

Fast Reinforcement Learning for Energy-Efficient Wireless Communication
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=5986747
*MATLAB-based simulation analysis*

Online Reinforcement Learning for Dynamic Multimedia Systems
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=5299114
*trace-based simulations*

INCdeep: Intelligent Network Coding with Deep Reinforcement Learning
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9488770
*Python 3.5-based framework, TensorFlow 1.15, to construct the architecture of INCdeep and its deep neural network*

Reinforcement Learning based ROI Bit Allocation for Gaming Video Coding in VVC
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9675345
*VVC Test Model and libtorch*

RL-AFEC: adaptive forward error correction for real-time video communication based on reinforcement learning
https://dl.acm.org/doi/pdf/10.1145/3524273.3528184
*To create the dataset for RL training, we concatenated videos in a random order to simulate a large video stream on the Internet.*

-------------------------------- ---------- --------------------------------




-------------------------------- Spectrum Access --------------------------------


Deep Multi-User Reinforcement Learning for Distributed Dynamic Spectrum Access
https://arxiv.org/pdf/1704.02613.pdf
Matlab

Deep Reinforcement Learning for Dynamic Multichannel Access in Wireless Networks
https://ieeexplore.ieee.org/abstract/document/8303773



==> old_unused_text.tex <==

% \section{Introduction}
% Numerous networking applications, such as traffic engineering, performance optimization, and network security, have witnessed a major uptick in the adoption of machine learning. Reinforcement learning has become an important trend among learning-based congestion control algorithms during the past decade \cite{badarla2011learning,jay2019deep, jin2018congestion, lan2019deep,li2016learning,li2018qtcp,mai2019self,nie2019dynamic,ramana2005learning,silva2016smart,,tarraf1995reinforcement,xiao2019tcp,xu2019experience, abbasloo2020classic}. Learning-based congestion control algorithms have the potential to adapt to a wide range of conditions without needing to be tuned or manually engineered for each one. This may eliminate the need for expensive human engineering and tuning for specific applications, which can be performed automatically by machines in shorter timeframes.

% However, learning-based CC is still in its infancy. When training a model with DRL, there are various design criteria to consider, including the action and state space, the reward function, the neural network model, and the DRL algorithm. The majority of learning-based CC algorithms regulate the sending rate by adjusting the congestion window \cite{badarla2011learning, lan2019deep,li2016learning,li2018qtcp,mai2019self,nie2019dynamic,ramana2005learning,silva2016smart,,tarraf1995reinforcement,xiao2019tcp,xu2019experience, abbasloo2020classic} as opposed to the sending rate itself \cite{jay2019deep, jin2018congestion}. Most techniques are primarily concerned with end-to-end CC when building the state space, employing a combination of signals derived from endpoint measurements, such as goodput, RTT, and inferred losses. In \cite{jay2019deep}  the state is defined as the derivative of latency with respect to time, the ratio of the current MI's mean latency to the shortest observable mean latency of any MI in the history of the connection, and the ratio of packets transmitted to packets recognised by the receiver. In \cite{xu2019experience} they employ goodput, average RTT, the mean deviation of RTTs, and CWND.  \cite{sacco2021owl} augments the state space with Partial Network Knowledge, a measure of the network's known congestion level, leveraging on in-network measurements. The reward definition can also vary significantly between designs: in \cite{abbasloo2020classic}  the reward function function is based on the well-studied metric of Power, but in \cite{jay2019deep}, the reward function is a linear combination of throughput, latency, and loss. 

% To determine the optimal policy, Reinforcement Learning control agents must engage in numerous interactions with the environment. Developing control algorithms and training them with simulation-generated data is often more practical than conducting testing in the real world, and it enables everyone to test their ideas without having to acquire and set up expensive testbeds. The agent's performance in the real world is contingent on the precision of the simulation models used during training. Since the scientific community strives to make its models as realistic as possible, simulation-based knowledge should also be applied to the real world. A standardised simulation-based framework also facilitate the reproducibility, examination, and expansion of results by others. In the absence of a standardised framework, RL solutions are often implemented in custom environments. In \cite{abbasloo2020classic}, models are trained on a pool of servers with a total of 320 CPU cores and edge-switches connected through high-speed links, with training and experimentation constrained by the real-time cost of transmitting data in a real network, in addition to the expensive cost of setting up the system. 

% In this paper, we introduce RayNet, a scalable and flexible reinforcement learning framework for network task resolution. Raynet combines the capability of carrying out large-scale network simulations in an efficient way by on of the de-facto event-based simulators used by the computer networks research community, Omnet++ \cite{}, and an open-source reinforcement learning library that supports highly distributed RL workloads while maintaining unified and simple APIs for a wide range of applications, Ray RLlib \cite{}. RLlib trains agents on environments that implement the OpenAI gym \cite{} environment's interface. As per our knowledge, this is the first publicly available implementation of an Omnet++ based OpenAI gym environment.

% \section{Related Work}
%  \cite{gawlowicz2019ns} proposed a training environment based on the ns-3 simulator \cite{}. While ns-3 performance in terms of memory usage and run-time simulation is slightly superior than that of Omnet++, Omnet++ provides a rich graphical user interface and an abstract modeling language, whereas ns-3 rely on pure source code for the development of the entire simulation \cite{weingartner2009performance}. \cite{fuhrer2022implementing} trained their RL models on an Omnet++ environemnt, but the training platform was not released. 



% I wouldn't really go down the way of competing with the ns-3 guys

%\section{Related Work}
 %\cite{gawlowicz2019ns} proposed a training environment based on the ns-3 simulator \cite{}. While ns-3 performance in terms of memory usage and run-time simulation is slightly superior than that of Omnet++, Omnet++ provides a rich graphical user interface and an abstract modeling language, whereas ns-3 rely on pure source code for the development of the entire simulation \cite{weingartner2009performance}. \cite{fuhrer2022implementing} trained their RL models on an Omnet++ environemnt, but the training platform was not released. 
 
%  We train a Receiver-Driven Congestion Control mechanism using RayNet. In Receiver Driven Protocols (RDP), the receiver controls the communication pace at the sender. Pull Requests (PR), which are small packets that, upon reception by the sender, trigger the delivery of a data packet, are used to control the transmission rate. Priority queues in switches are used to convey PRs. When data packet queues overflow, packets are trimmed rather than dropped, and trimmed headers are delivered to the receiver using priority queues, informing the receiver that congestion-related packet loss has occurred.
% RDPs have exhibited outstanding performance in specific networking environments, such as data centres. RDP implementations are restricted to flow control and optimised for the receiver's physical link, which is expected to be the bottleneck of any incoming connection. Adding a congestion control mechanism to a receiver-driven protocol would permit the deployment of an RDP in networks where there may be bottlenecks in other parts of the connection's path and in networks where the receive link is unknown in advance. Packet Trimming provides the receiver with explicit and timely congestion indications, whereas PRs permit the receiver to change the transmission rate as soon as a congestion is identified.

==> programming_snippet.tex <==


% \textcolor{teal}{Every step event in the simulation loop triggers a set of virtual methods used to fetch observations and rewards from the agent and pass the action on to the next step. The implementation of each function must be provided by the programmer as it is specific to each use case.}

% \begin{lstlisting}[language=C++]
% class RLInterface {
%     virtual ObsType getObs() = 0;
%     virtual RewardType getReward() = 0;
%     virtual bool getDone() = 0;
%     virtual bool setAction(ActionType action) = 0;
% }
% \end{lstlisting}

% \textcolor{teal}{The resetting and stepping logic of the simulation model are exported to a Python module using python bindings. The programmer can import this module and interact with the underling simulation module by instantiating an object from the exported \textit{GymApi} class and by calling its methods:}

% \begin{lstlisting}[language=C++]
% py::class_<GymApi>(m, "OmnetGymApi")
%     .def(py::init<>())
%     .def("initialise", &GymApi::initialise)
%     .def("reset", &GymApi::reset)
%     .def("step", &GymApi::step)
%     .def("shutdown", &GymApi::shutdown)
%     .def("cleanup", &GymApi::cleanupmemory);
% \end{lstlisting}

% \textcolor{teal}{This feature seamlessly integrates with any python script, enabling the creation of a custom Python class environment:}

% \begin{lstlisting}[language=Python]
% class OmnetGymApiEnv(gym.Env):
%     def __init__(self):
%         self.action_space = spaces.Box()
%         self.observation_space = spaces.Box()
%         self.gym_api = OmnetGymApi()  # Python bindings module

%     def reset(self, *, seed=None, options=None):
%         # Custom simulation configuration code
%         sim_config = prepare_sim_config(seed)
%         self.gym_api.initialise(sim_config)
%         obs = self.gym_api.reset()
%         # Tailored raw observation processing, e.g., stacking, masking
%         return obs

%     def step(self, action):
%         obs, rewards, dones, info = self.gym_api.step(actions)
%         if dones[self.agentId]:
%             self.gym_api.shutdown()
%             self.gym_api.cleanup()
%         return obs, reward, dones[self.agentId], False, {}
% \end{lstlisting}

% \textcolor{teal}{In this example, notice the encapsulation of the Python binding module within the \textit{OmnetGymApiEnv} class. This encapsulation allows for the extension of the basic functionality provided by the Python module. For instance, the reset method in \textit{OmnetGymApiEnv} can handle the initialization of simulation configuration parameters by drawing random values from custom distributions, and it can stack consecutive observations into a fixed-length frame. The \textit{OmnetGymApiEnv} is then passed to Ray as a custom OpenAI gym environment.}

